Normalized Augmented Inverse Probability Weighting with Neural Network Predictions

The estimation of Average Treatment Effect (ATE) as a causal parameter is carried out in two steps, where in the first step, the treatment and outcome are modeled to incorporate the potential confounders, and in the second step, the predictions are inserted into the ATE estimators such as the Augmented Inverse Probability Weighting (AIPW) estimator. Due to the concerns regarding the nonlinear or unknown relationships between confounders and the treatment and outcome, there has been an interest in applying non-parametric methods such as Machine Learning (ML) algorithms instead. Some literature proposes to use two separate Neural Networks (NNs) where there's no regularization on the network's parameters except the Stochastic Gradient Descent (SGD) in the NN's optimization. Our simulations indicate that the AIPW estimator suffers extensively if no regularization is utilized. We propose the normalization of AIPW (referred to as nAIPW) which can be helpful in some scenarios. nAIPW, provably, has the same properties as AIPW, that is, the double-robustness and orthogonality properties. Further, if the first step algorithms converge fast enough, under regulatory conditions, nAIPW will be asymptotically normal. We also compare the performance of AIPW and nAIPW in terms of the bias and variance when small to moderate L1 regularization is imposed on the NNs.

==> Influence_curve.tex <==

\iffalse
which is upper bounded by the following
\begin{equation}
    \sqrt{n}\Bigg[\mathbb{E}\Big[\frac{g}{\hat{g}\mathbb{E}\frac{A}{\hat{g}}}-1\Big]^p\Bigg]^{\frac{1}{p}}\Bigg[\mathbb{E}\Big[Q^1-\hat{Q}^1\Big]^q\Bigg]^{\frac{1}{q}}
\end{equation}
by the h\"older's inequality, for $p$ and $q$ such that $\frac{1}{p}+\frac{1}{q}=1$. By this formula, either of the estimated outcome or propensity score prediction models can converge slower than (like $n^{-\frac{1}{p}}$ where $p>2$) while the other converges faster than $\frac{1}{\sqrt{n}}$(like $n^{-\frac{1}{q}}$ where $q<2$) as long as the summation of their rates equals $\frac{1}{\sqrt{n}}$.
\fi








{\bf Efficient Influence Curve}

For the following content, we use the notations and results of \cite{hines2021demystifying} for calculating the Efficient Influence Curve of nAIPW. Let $P$ be the data generating process law.

\begin{equation}
    \Psi(P) = \frac{\mathbb{E}_P[\mathbb{E}_P[Y|A=1,W]]}{\mathbb{E}_P[\frac{A}{g}]} := \frac{\Phi(P)}{\Omega(P)},
\end{equation}
that is, $\Phi(P)=\mathbb{E}_P[\mathbb{E}_P[Y|A=1,W]]$ is the AIPW estimator and $\Omega(P)=\mathbb{E}_P[\frac{A}{g}]$ is the normalizing term.

The efficient influence curve is the path-wise derivative of $\Psi(P_t)=t\Psi(\tilde{P})+(1-t)\Psi(P)$:

\begin{equation}
    \frac{\partial \Psi(P_t)}{\partial t}\Big|_{t=0} = \frac{\frac{\partial \Phi(P_t)}{\partial t}\Big|_{t=0}\Omega(P)-\frac{\partial \Omega(P_t)}{\partial t}\Big|_{t=0}\Phi(P)}{\Omega(P)^2}
\end{equation}
where $\Phi(P_t)=t\Phi(\tilde{P})+(1-t)\Phi(P)$ and $\Omega(P_t)=t\Omega(\tilde{P})+(1-t)\Omega(P)$. Further, from \cite{hines2021demystifying} we have that
\begin{equation}
    \frac{\partial \Phi(P_t)}{\partial t}\Big|_{t=0} = \frac{A}{g}(Y-Q^1)+Q^1-\Phi(P).
\end{equation}

Also, by definition of $\Omega$, the standard regulatory conditions that the derivative goes inside the integral, and the fact that $\mathbb{E}_P[A=1|W=w]=f(1|w)=\frac{f(1,w)}{f(w)}$,
\begin{multline}
    \frac{\partial \Omega(P_t)}{\partial t}\Big|_{t=0} = \int \frac{\partial}{\partial t} \frac{Af_t(w)}{\mathbb{E}_P[A=1|W]} \ \  dw=\int \frac{\partial}{\partial t} \frac{Af_t(w)}{f_t(1|w)} \ \  dw=\int \frac{\partial}{\partial t} \frac{Af_t^2(w)}{f_t(1,w)} \ \  dw=\\ \int A \frac{2f(w)f(1,w)f'_{t=0}(w)-f^2(w)f'_{t=0}(1,w)}{f^2(1,w)} \ \  dw.
\end{multline}
Again in \cite{hines2021demystifying} it is shown that the path-wise derivative of the density $f$ on $o$ toward $\tilde{o}$ is:
\begin{equation}
    f'_{t=0}(o) = I_o(\tilde{o}) - f(o),
\end{equation}
for observation $o$, which can be one or more than one dimensional.  Thus 
\begin{multline}
    \frac{\partial \Omega(P_t)}{\partial t}\Big|_{t=0} =  \int A \frac{2f(w)f(1,w)\big(I_w(\tilde{w})-f(w)\big)-f^2(w)\big(I_{a,w}(\tilde{a},\tilde{w})-f(1,w)\big)}{f^2(1,w)} \ \  dw\\
    \int \frac{A}{f^2(1,w)} \Big[2f(w)f(1,w)I_w(\tilde{w})-2f^2(w)f(1,w)-I_{a,w}(\tilde{a},\tilde{w})f^2(w)+f^2(w)f(1,w)\Big] \ \ dw \\
    2\int \frac{Af(\tilde{w})}{f(1,\tilde{w})} \ \ dw -2 \int \frac{Af^(w)}{f(1,w)} \ \ dw-\int A \frac{f^2(\tilde{w})}{f^2(1,\tilde{w})}  \ \ dw+ \int \frac{Af(w)}{f(1,w)} \ \ dw = \\
    \frac{2A}{f(1|\tilde{w})}-2\Omega(P)-\frac{A}{f^2(1|\tilde{w})}+\Omega(P)=\frac{A}{g}(2-\frac{1}{g})-\Omega(P),
\end{multline}
where in the last equality we can replace $\tilde{w}$ with observed data. Hence,

\begin{multline}
\frac{\partial \Psi(P_t)}{\partial t}\Big|_{t=0} = \frac{1}{\Omega^2} \Big[ \Omega\big( \frac{A}{g}(Y-Q^1)+Q^1-\Phi \big) - \Phi \big( \frac{A}{g}(2-\frac{1}{g})-\Omega \big)\Big] =\\ \frac{A(Y-Q^1)}{g\mathbb{E}[\frac{A}{g}]}-\frac{Q^1}{\mathbb{E}[\frac{A}{g}]}-\frac{A\Phi(2-\frac{1}{g})}{g\mathbb{E}^2[\frac{A}{g}]}
\end{multline}

Then, the efficient influence function of nAIPW estimator is:

\begin{equation}
EIF_{nAIPW}=\Big(\frac{A(Y-Q^1)}{g\mathbb{E}[\frac{A}{g}]}-\frac{(1-A)(Y-Q^0)}{(1-g)\mathbb{E}[\frac{1-A}{1-g}]}\Big)+\Big(\frac{Q^1}{\mathbb{E}[\frac{A}{g}]}-\frac{Q^0}{\mathbb{E}[\frac{1-A}{1-g}]}\Big)-\Big(\frac{A(2-\frac{1}{g})\Phi^1}{g\mathbb{E}^2[\frac{A}{g}]}-\frac{(1-A)(2-\frac{1}{1-g})\Phi^0}{(1-g)\mathbb{E}^2[\frac{1-A}{1-g}]}\Big),
\end{equation}
where $\Phi$ is the AIPW estimator. Notice that for an experimental design with $P(A=1|W)=\frac{1}{2}$, the third component vanishes.

Comparing it to the efficient influence function of AIPW
\begin{equation}
    EIF_{AIPW}=\Big(\frac{A(Y-Q^1)}{g}-\frac{(1-A)(Y-Q^0)}{1-g}\Big)+\Big(Q^1-Q^0\Big)-\Phi.
\end{equation}


\iffalse
\[ EIF_{nAIPW}=\begin{cases} 
      \frac{Y^1-Q^1}{g\mathbb{E}[\frac{A}{g}]}-\frac{(2g-1)(Y^1-Q^1)}{g^3\mathbb{E}^2[\frac{A}{g}]}+\frac{Q^1}{\mathbb{E}[\frac{A}{g}]} & \qquad  A=1, \\ \\
      -\frac{Y^0-Q^0}{(1-g)\mathbb{E}[\frac{1-A}{1-g}]}+\frac{(1-2g)(Y^0-Q^0)}{(1-g)^3\mathbb{E}^2[\frac{1-A}{1-g}]}-\frac{Q^0}{\mathbb{E}[\frac{1-A}{1-g}]} & \qquad  A=0,
   \end{cases}
\]
or
\[ EIF_{nAIPW}=\begin{cases} 
      \frac{Y^1-Q^1}{g\mathbb{E}[\frac{A}{g}]}\Big(1+\frac{1-2g}{g^2\mathbb{E}[\frac{A}{g}]}\Big)+\frac{Q^1}{\mathbb{E}[\frac{A}{g}]} & \qquad  A=1, \\ \\
      -\frac{Y^0-Q^0}{(1-g)\mathbb{E}[\frac{1-A}{1-g}]}\Big(1+\frac{2g-1}{(1-g)^2\mathbb{E}[\frac{1-A}{1-g}]}\Big)-\frac{Q^0}{\mathbb{E}[\frac{1-A}{1-g}]} & \qquad  A=0.
   \end{cases}
\]
\[ EIF_{AIPW}=\begin{cases} 
      \frac{Y^1-Q^1}{g}+Q^1-\Phi^1 & \qquad  A=1, \\ \\
      -\frac{Y^0-Q^0}{1-g}-Q^0+\Phi^0 & \qquad  A=0,
   \end{cases}
\]
we see that
\fi








In nAIPW, however, we are proposing to create a slightly different estimator:
\begin{multline}
    \sqrt{n}(\hat{\beta}+\frac{1}{\sqrt{n}}\phi(O, \hat{P}_n)-\beta) =
    \\ \sqrt{n}\Big(\frac{1}{n}\sum_{i=1}^n\Big[\frac{A_i}{g_i\frac{1}{n}\sum_{i=1}^n\frac{A_i}{g_i}}(Y_i-\hat{Q}_i^1)-\frac{1-A_i}{(1-g_i)\frac{1}{n}\sum_{i=1}^n\frac{1-A_i}{1-g_i}}(Y_i-\hat{Q}_i^0)+\hat{Q}_i^1-\hat{Q}_i^0\Big]-\beta\Big)=\\
    (first+third+forth)+\Big(\frac{1}{\sqrt{n}}\sum_{i=1}^n\frac{A_i}{g_i}(Y_i-\hat{Q}_i^1)\Big)\Big(\frac{n}{\sum_{i=1}^n\frac{A_i}{g_i}}-1\Big)-
    \\\Big(\frac{1}{\sqrt{n}}\sum_{i=1}^n\frac{1-A_i}{1-g_i}(Y_i-\hat{Q}_i^0)\Big)\Big(\frac{n}{\sum_{i=1}^n\frac{1-A_i}{1-g_i}}-1\Big).
\end{multline}
The $first, third, forth$ terms refer to the first, third, and forth terms on \eqref{taylor}. If the true values of the propensity scores $g$ were known, the extra terms would vanish. If $g$ is unknown and we replace it with data adaptive $\hat{g}$, as $\mathbb{E}[\frac{A}{g}]=1$, the extra terms can vanish as long as $\hat{g}\xrightarrow{p}g$. The main challenge arises when the positivity assumption is violated due to small sample sizes \citep{van2011targeted}.

==> benchmark_resuls.tex <==

% In this section we apply the two-step causal inference 

% \subsection{Benchmark Datasets}

% The IBM causal inference benchmarking framework \citep{shi2019adapting}, derived from the LBIDD dataset, the Births and Infant Deaths Database \citep{macdorman1998infant}. The IBM benchmarking datasets contain data of the birth and infant death certificates registered in all States and the District of Columbia. The input features are obtained from the same observed inputs (including the treatment) in the original LBIDD dataset, but the outcomes are generated based on different generating processes with different non-linearities introduced. Different generating processes result in different datasets and the truth for the individual observed and counterfactuals outcomes and thus for the true ATE are known. This set of datasets is one of the standard tools for comparison purposes \citep{shalit2017estimating}.

% Figures \ref{benchmarks-figs} illustrate the results of DR and nDR and their 95\% asymptotic confidence intervals for 15 different benchmark datasets, and for 3 different Neural Network hyperparameter settings. The true average effects for each dataset are shown in dots. Generally, the confidence intervals of nAIPW is shorter or as wide as that of AIPW. The first step predictions are calculated using the dNN method, with 3 hidden layers with the same size as the number of inputs. Three different values for the $L_1$ regularization determines the three different hyperparameter settings. 


% \begin{figure}[ht!]
% \centering
% \caption{Results of DR and nDR and their 95\% confidence intervals for 15 different benchmark datasets, and the true effects in each dataset. Note generally wider CIs and more bias (distance from the truth) in case of no regularization. nDR is always superior or non-inferior to DR. }
% \includegraphics[scale=0.55]{benchmarks-Oct2021.pdf}
% \label{benchmarks-figs}
% \end{figure}

%compare summations/normalizations with n. 
% Check 1/ps for different scenarios, for cchs
% Add IPW as well. 
% Must numerically check why intervals are wide, but not in simulations


==> orthogonality_proof.tex <==
\begin{multline}\label{nAIPWorthog}
   \partial_{\eta} \mathbb{E}_P \phi\big(\mathbf{O}, \beta, \eta\big)\Big|_{\eta=\eta_0} [\eta-\eta_0] = \partial_{\eta} \mathbb{E}_P\Big(Q^1-Q^0-\beta + \frac{A(Y^1-Q^1)}{g\mathbb{E}\big(\frac{A}{g}\big)} - 
   \frac{(1-A)(Y^0-Q^0)}{(1-g)\mathbb{E}\big(\frac{1-A}{1-g}\big)}\Big)|_{\eta=\eta_0} [\eta-\eta_0]\propto\\ \mathbb{E}_P \Big(1-\frac{A}{g\mathbb{E}\big(\frac{A}{g}\big)}, \ -1+\frac{1-A}{(1-g)\mathbb{E}\big(\frac{1-A}{1-g}\big)}, \ A(Y^1-Q^1)f_1(g)+(1-A)(Y^0-Q^0)f_2(g)\Big)\Big|_{\eta=\eta_0},
\end{multline}



Note that AIPW and nAIPW do not require the same adjustment covariate set to be used in both the propensity score model and the outcome model \citep{glynn2010introduction, pearl1995causal, winship2007counterfactuals}. The requirement is that the above identifiability assumptions hold given covariates. This flexibility allows the researcher to, for instance, use the minimal set of adjustment variables necessary for conditional ignorability to hold in the propensity score model while including a near maximal set of adjustment variables in the outcome regression models. 










In a worst case scenario assume $g_j=10^t$, where $j\in I_k$, and $g_k=10^s$ where $t \gg s$, one might argue that normalization might not be help. In this case a similar argument can made to see the more stability of nAIPW:

\begin{equation}\label{scen21}
    \beta_{1, AIPW} = \frac{1}{n}\Big(10^s(Y_k-Q^1_k)+\sum_{i\in I_{-k} }(Y_i-Q^1_i)10^t\Big)+\frac{1}{n}\sum_{i=1}^nQ^1_i,
\end{equation}
and given that $|I_{-k}|$ is the number of observations in the treatment group ($A=1$) which are not equal to $k^{th}$ observation,
\begin{multline}\label{scen22}
    \beta_{1, nAIPW} = \Big(\frac{Y_k-Q^1_k}{10^{-s}(\frac{1}{10^{-s}}+\frac {|I_{-k}|}{10^{-t}})}+\sum_{i\in I_{-k} }\frac{Y_i-Q^1_i}{10^{-t}(\frac{1}{10^{-s}}+\frac{|I_{-k}|}{10^{-t}})}\Big)+\beta_{SR}=\\ 
    \Big(\frac{Y_k-Q^1_k}{(1+|I_{-k}|10^{s-t})}+\sum_{i\in I_{-k} }\frac{Y_i-Q^1_i}{10^{s-t}+|I_{-k}|}\Big)+\frac{1}{n}\sum_{i=1}^nQ^1_i,
\end{multline}
where the first term in right hand side is finite and the terms in the summations \eqref{scen22} are smaller than those in \eqref{scen21}. Similar arguments hold in the average untreated group which indicates that nAIPW is more robust to extreme predictions of the propensity scores than AIPW, and thus the loss. 

